Cosmos-Transfer1: Conditional World Generation with Adaptive Multimodal Control

We introduce Cosmos-Transfer, a conditional world generation model that can generate world simulations based on multiple spatial control inputs of various modalities such as segmentation, depth, and edge. In the design, the spatial conditional scheme is adaptive and customizable. It allows weighting different conditional inputs differently at different spatial locations. This enables highly controllable world generation and finds use in various world-to-world transfer use cases, including Sim2Real. We conduct extensive evaluations to analyze the proposed model and demonstrate its applications for Physical AI, including robotics Sim2Real and autonomous vehicle data enrichment. We further demonstrate an inference scaling strategy to achieve real-time world generation with an NVIDIA GB200 NVL72 rack. To help accelerate research development in the field, we open-source our models and code at https://github.com/nvidia-cosmos/cosmos-transfer1.

==> figures/1_introduction/fig_cosmos_transfer_architecture.tex <==
\begin{figure*}[t!]
\centering
    \includegraphics[width=0.8\textwidth]{images/1_introduction/cosmos_transfer_architecture.pdf}
    \caption{{\bf Overview of the architecture of Cosmos-Transfer1.} We train individual ControlNets separately for each sensor modality used to capture the simulated world. At inference time, the control signals from each control branch are multiplied by their corresponding adaptive spatiotemporal control maps and then summed before being added to the transformer blocks of the base model. We use the adaptive spatiotemporal control maps to allow the model to leverage the most relevant modalities in different regions for optimal output quality.}
    \label{fig:arch}
\end{figure*}

==> figures/backup/cosmos_transfer_diagram.tex <==
\begin{figure*}[h]
\centering
    \includegraphics[width=0.8\textwidth]{figures/cosmos_transfer.pdf}
    \caption{Cosmos-Transfer1 adaptively fuses complementary simulated world representations into a unified physical world, enabling scalable synthesis of diverse and robust real-world data that captures intricate physical complexities and dynamics.}
    \label{fig:cosmos_transfer_diagram}
\end{figure*}

==> figures/backup/ctrlnets_part2.tex <==
\begin{figure*}[h]
\centering
    \includegraphics[width=0.99\textwidth]{figures/ctrlnets_part2.pdf}
    \caption{...}
    \label{fig:ctrlnets_part2}
\end{figure*}
